Progressive Gradient Flow for Robust N:M Sparsity Training in Transformers

N:M Structured sparsity has garnered significant interest as a result of relatively modest overhead and improved efficiency. Additionally, this form of sparsity holds considerable appeal for reducing the memory footprint owing to their modest representation overhead. There have been efforts to develop training recipes for N:M structured sparsity, they primarily focus on low-sparsity regions ($\sim$50\%). Nonetheless, performance of models trained using these approaches tends to decline when confronted with high-sparsity regions ($>$80\%). In this work, we study the effectiveness of existing sparse training recipes at \textit{high-sparsity regions} and argue that these methods fail to sustain the model quality on par with low-sparsity regions. We demonstrate that the significant factor contributing to this disparity is the presence of elevated levels of induced noise in the gradient magnitudes. To mitigate this undesirable effect, we employ decay mechanisms to progressively restrict the flow of gradients towards pruned elements. Our approach improves the model quality by up to 2$\%$ and 5$\%$ in vision and language models at high sparsity regime, respectively. We also evaluate the trade-off between model accuracy and training compute cost in terms of FLOPs. At iso-training FLOPs, our method yields better performance compared to conventional sparse training recipes, exhibiting an accuracy improvement of up to 2$\%$. The source code is available at https://github.com/abhibambhaniya/progressive_gradient_flow_nm_sparsity.

==> Sections/09-Checklist.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on answering these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Tables/ab_update_freq.tex <==
\begin{table}[t]\centering
\caption{The effect of update frequency in SR-STE~\citep{sr_ste}. Raising the ``Update Frequency'' increases the training time significantly. Hence, we only include the results for ``Update Frequency'' 100 and 1000.}
\scriptsize
\begin{tabular}{lrrrr}\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Accuracy}} &\multicolumn{2}{c}{Update Frequency} \\\cmidrule{3-4}
& &every 1000 steps &every 100 steps \\\midrule
\multirow{4}{*}{Sparsity Target} &1:16 &0.709 &0.710 \\
&1:32 &0.707 &0.707 \\
&1:64 &0.706 &0.706 \\
&1:128 &0.706 &0.706 \\
\bottomrule
\end{tabular}
\label{table:ab_update_freq}
\end{table}

==> Tables/ablation_decay_rate.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Ablation: The effect of mask decay rate ($\beta^t$).}
\scriptsize
\begin{tabular}{lrrrrrr}\toprule
\multicolumn{2}{c}{Accuracy} &\multicolumn{4}{c}{Mask Decay} \\\cmidrule{1-6}
\multicolumn{2}{c}{Sparsity Target} &1:16 &1:32 &1:64 &1:128 \\\midrule
\multirow{2}{*}{Mask decay rate ($\beta^t$)} &0.9 &\textbf{0.715} &\textbf{0.713} &\textbf{0.711} &\textbf{0.710} \\
&0.001 &0.712 &0.709 &0.708 &0.707 \\
\bottomrule
\end{tabular}
\label{table:ab_decay_rate}
\end{table}

==> Tables/ablation_exp_decay_rate.tex <==
\begin{table}[!htp]\centering
\caption{Ablation: The effect of mask decay rate ($\beta^t$) for \mdgf-Exponential.}
\scriptsize
\begin{tabular}{lr|rrrr}\toprule
% \multicolumn{2}{c}{Accuracy} &\multicolumn{4}{c}{Mask Decay} \\\cmidrule{1-6}
Mask decay rate & ($\beta^t$)  & 1e-3 & 1e-4 & 5e-5 & 1e-5 \\\midrule
Sparsity Target & 1:4 &\textbf{78.579} &78.403 &78.157 &76.477 \\
% &0.001 &0.712 &0.709 &0.708 &0.707 \\
\bottomrule
\end{tabular}
\label{table:exp_decay_ablation}
\end{table}


==> Tables/ablation_srste.tex <==
\begin{table*}[!htp]\centering
\caption{Ablation: SR-STE augmented with few epochs of dense training.}
\scriptsize
\begin{tabular}{lrrrrrrr}\toprule
&\multicolumn{2}{c}{Training Schedule} &\multicolumn{4}{c}{Accuracy} \\\cmidrule{2-7}
&Dense steps &SR-STE -styled Sparse steps &1:16 &1:32 &1:64 &1:128 \\\cmidrule{2-7}
SR-STE &0 &200K &0.710 &0.707 &0.706 &0.706 \\\midrule
\multirow{4}{*}{Dense + SR-STE} &2.5K &197.5K &0.712 &0.710 &\textbf{0.708} &0.706 \\
&5K &195K &0.712 &0.709 &0.707 &\textbf{0.708} \\
&10K &190K &0.712 &\textbf{0.710} &0.707 &\textbf{0.708} \\
&20K &180K &\textbf{0.713} &\textbf{0.710} &\textbf{0.708} &0.707 \\
\bottomrule
\end{tabular}
\label{table:ab_srste}
\end{table*}

==> Tables/compare_flops.tex <==
\begin{table*}[!t]\centering
\caption{The comparisons of the training recipes performance (Inference FLOPs) and model accuracy (Top-1).
%
We compare dense model with iso-inference flops and iso-accuracy sparse models between SR-STE and our decaying-based methods, \mdgf and \sdgf.}
\scriptsize
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}\toprule
Model & Sparsity recipe &Sparsity Target & Top-1 Acc~(\%) $\uparrow$ & Param~(M) $\downarrow$ & Inference FLOPs~(G)$\downarrow$\\\midrule
\xx{ViT-Base} & - & Dense & 76.389 & 86.23 (100\%)  &  34.71 (100\%) \\ 
\midrule
% \xx{ViT-Base} & SR-STE & 1:16 (FF) & 75.637 & 33.15 (38.5\%)  & 13.9 (40\%) \\
% \xx{ViT-Base} & \mdgf-Exp & 1:16 (FF) & 77.325 & 33.15 (38.5\%)  & 13.9 (40\%) \\ 
% \midrule
% \xx{ViT-Base} & SR-STE & 1:8 (FF)  & 77.869 & 36.68 (42.5\%)  & 15.3 (44\%) \\
% \xx{ViT-Base} & \sdgf-Geometric & 1:8 (FF) & 78.175 & 36.68 (42.5\%)  & 15.3 (44\%) \\
% \midrule
% \xx{ViT-Base} & SR-STE & 1:8 (FF) + 1:8 (QK)  & 75.527 & 24.3 (28.1\%) & 10.4 (30\%) \\
% \xx{ViT-Base} & \mdgf-Exp & 1:8 (FF) + 1:8 (QK) & 77.349 & 24.3 (28.1\%) & 10.4 (30\%) \\

\midrule
\xx{ViT-Base} & SR-STE & 1:16 (FF) & 75.637 & 33.15 (38.5\%)  & 13.9 (40\%) \\
\xx{ViT-Base} & \mdgf-Exp & 1:32 (FF) & 76.068 &  \\ 
\midrule
\xx{SwinV2-Base} & SR-STE & 1:8 (FF)  & 77.869 & 36.68 (42.5\%)  & 15.3 (44\%) \\
\xx{ViT-Base} & \sdgf-Geometric & 1:8 (FF) & 78.175 & 36.68 (42.5\%)  & 15.3 (44\%) \\
\midrule
\xx{ViT-Base} & SR-STE & 1:8 (FF) + 1:8 (QK)  & 75.527 & 24.3 (28.1\%) & 10.4 (30\%) \\
\xx{ViT-Base} & \mdgf-Exp & 1:8 (FF) + 1:8 (QK) & 77.349 & 24.3 (28.1\%) & 10.4 (30\%) \\
\bottomrule
\end{tabular}
% }
\label{table:cpr_flops}
\end{table*}




==> cross_ent_loss_t5x_plots/cross_ent_loss_t5x_plots.tex <==
\begin{figure*}[!hbt]
   \centering
\subfigure[1:4 (FF)]{\label{cross_ent_loss_t5x:1_4_ff}
\includegraphics[width=0.45\linewidth]{cross_ent_loss_t5x_plots/cross_ent_loss_1_4_ff.pdf}}
\subfigure[1:32 (FF)]{\label{cross_ent_loss_t5x:1_32_ff}
\includegraphics[width=0.45\linewidth]{cross_ent_loss_t5x_plots/cross_ent_loss_1_32_ff.pdf}}\\
\subfigure[1:8 (FF+QK)]{\label{cross_ent_loss_t5x:1_8_ffqk}
\includegraphics[width=0.45\linewidth]{cross_ent_loss_t5x_plots/cross_ent_loss_1_8_ffqk.pdf}}
\subfigure[1:8 (FF+QKV)]{\label{cross_ent_loss_t5x:1_8_ffqkv}
\includegraphics[width=0.45\linewidth]{cross_ent_loss_t5x_plots/cross_ent_loss_1_8_ffqkv.pdf}}\\
\subfigure[1:8 (FF)+1:4 (QKV)]{\label{cross_ent_loss_t5x:1_8_ff_1_4_qkv}
\includegraphics[width=0.45\linewidth]{cross_ent_loss_t5x_plots/cross_ent_loss_1_8_ff_1_4_qkv.pdf}}
\caption{Cross entropy loss for \xx{T5X-Base} model finetuned on the GLUE dataset for 50\,K steps.\ay{cut it to 1.05}}
\label{fig:cross_ent_loss_t5x}
\end{figure*}

==> eval_t5x_plots_1_8_ff_1_4_qkv/eval_t5x_plots.tex <==
\begin{figure*}[!hbt]
   \centering
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:cola}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_cola_v002_eval_matthews_corrcoef_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:mnli_matched}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_mnli_matched_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:mnli_mismatched}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_mnli_mismatched_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}\\
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:mrpc:accuracy}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_mrpc_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:mrpc:f1}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_mrpc_v002_eval_f1_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:qnli}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_qnli_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}\\
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:qqp:accuracy}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_qqp_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:qqp:f1}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_qqp_v002_eval_f1_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:rte}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_rte_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}\\
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:sst2}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_sst2_v002_eval_accuracy_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:stsb:pearson_corr}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_stsb_v002_eval_pearson_corrcoef_1_8_ff_1_4_qkv.pdf}}
%
\subfigure{\label{eval_t5x_1_8_ff_1_4_qkv:stsb:spearman}
\includegraphics[width=0.32\linewidth]{eval_t5x_plots_1_8_ff_1_4_qkv/glue_stsb_v002_eval_spearman_corrcoef_1_8_ff_1_4_qkv.pdf}}
\caption{\ay{fill later}.}
\label{fig:eval_t5x_1_8_ff_1_4_qkv}
\end{figure*}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

